Graph Neural Networks for Forecasting Multivariate Realized Volatility with Spillover Effects

We present a novel methodology for modeling and forecasting multivariate realized volatilities using customized graph neural networks to incorporate spillover effects across stocks. The proposed model offers the benefits of incorporating spillover effects from multi-hop neighbors, capturing nonlinear relationships, and flexible training with different loss functions. Our empirical findings provide compelling evidence that incorporating spillover effects from multi-hop neighbors alone does not yield a clear advantage in terms of predictive accuracy. However, modeling nonlinear spillover effects enhances the forecasting accuracy of realized volatilities, particularly for short-term horizons of up to one week. Moreover, our results consistently indicate that training with the Quasi-likelihood loss leads to substantial improvements in model performance compared to the commonly-used mean squared error. A comprehensive series of empirical evaluations in alternative settings confirm the robustness of our results.

==> tables/longer_horizon.tex <==
\begin{tabular}{lcccccccc}
\toprule
& \multicolumn{4}{c}{1-Week} & \multicolumn{4}{c}{{1-Month}} \\
     \cmidrule(lr){2-5}\cmidrule(lr){6-9}
& \multicolumn{2}{c}{{MSE}} & \multicolumn{2}{c}{{QLIKE}} & \multicolumn{2}{c}{{MSE}} & \multicolumn{2}{c}{{QLIKE}} \\
     \cmidrule(lr){2-3}\cmidrule(lr){4-5} \cmidrule(lr){6-7}\cmidrule(lr){8-9}
 & Ratio  & $p$-val &  Ratio & $p$-val  & Ratio  & $p$-val &  Ratio & $p$-val \\
\midrule
% \multicolumn{5}{c}{Panel A: trained with MSE} \\\midrule
HAR$_M$           & 1.000 & $<$0.001  & 1.000 & $<$0.001  & 1.000 & 0.003   & 1.000 & $<$0.001  \\
GHAR$_M$          & 0.904 & $<$0.001  & 0.987 & $<$0.001  & 0.975 & 1.000   & 1.036 & $<$0.001  \\
GNNHAR1L$_M$      & 0.940 & $<$0.001  & 0.943 & $<$0.001  & 1.021 & 0.003   & 0.968 & 0.001   \\
GNNHAR2L$_M$      & 1.034 & $<$0.001  & 0.953 & $<$0.001  & 1.134 & $<$0.001  & 1.032 & $<$0.001  \\
GNNHAR3L$_M$      & 1.014 & $<$0.001  & 0.961 & $<$0.001  & 1.046 & $<$0.001  & 0.958 & 0.011   \\\midrule
HAR$_Q$           & 0.939 & $<$0.001  & 0.945 & $<$0.001  & 1.069 & $<$0.001  & 0.986 & $<$0.001  \\
GHAR$_Q$          & 0.842 & 1.000   & 0.936 & $<$0.001  & 1.151 & $<$0.001  & 0.954 & 0.015   \\
GNNHAR1L$_Q$      & 0.855 & $<$0.001  & 0.913 & 1.000   & 1.179 & $<$0.001  & 0.965 & 0.001   \\
GNNHAR2L$_Q$      & 0.933 & $<$0.001  & 0.92  & 0.003   & 1.736 & $<$0.001  & 0.927 & 1.000   \\
GNNHAR3L$_Q$      & 1.185 & $<$0.001  & 0.942 & $<$0.001  & 1.502 & $<$0.001  & 0.971 & $<$0.001  \\
\bottomrule
\end{tabular}


==> tables/regime1.tex <==
\begin{tabular}{lllllll}
\toprule
 & \multicolumn{2}{c}{{1-Day}} & \multicolumn{2}{c}{{1-Week}} & \multicolumn{2}{c}{{1-Month}}  \\
     \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
                 & MSE    & QLIKE  & MSE    & QLIKE  & MSE     & QLIKE  \\\midrule
                 & \multicolumn{6}{c}{{Panel A: Bottom 90\%}}  \\ \midrule
HAR$_M$          & 1.000   & 1.000  & 1.000  & 1.000  & 1.000   & 1.000  \\
GHAR$_M$         & 0.961   & 0.998   & 0.949  & 1.001   & 0.967   & 1.027   \\
GNNHAR1L$_M$     & 0.943$^*$  & 0.998   & 0.883$^*$ & 0.960$^{\dagger}$  & 0.923$^*$  & 0.924$^{\dagger}$ \\
GNNHAR2L$_M$     & 0.944$^{\dagger}$ & 0.990   & 0.901  & 0.954$^{\dagger}$ & 0.946$^{\dagger}$ & 0.921$^*$  \\
GNNHAR3L$_M$     & 0.957   & 0.987   & 0.911  & 0.965   & 0.937$^{\dagger}$ & 0.930$^{\dagger}$ \\
HAR$_Q$          & 1.010   & 0.984   & 1.005  & 0.955$^{\dagger}$ & 1.159   & 0.942$^{\dagger}$ \\
GHAR$_Q$         & 0.989   & 1.007   & 1.076  & 1.001   & 1.257   & 1.084   \\
GNNHAR1L$_Q$     & 0.967   & 0.978$^*$  & 0.944  & 0.943$^*$  & 1.478   & 0.977   \\
GNNHAR2L$_Q$     & 0.976   & 0.979$^{\dagger}$ & 0.985  & 0.947$^{\dagger}$ & 1.433   & 0.973   \\
GNNHAR3L$_Q$     & 0.970   & 0.980$^{\dagger}$ & 1.062  & 0.957   & 1.662   & 0.969   \\
\bottomrule
\end{tabular}

==> tables/regime2.tex <==
\begin{tabular}{lllllll}
\toprule
 & \multicolumn{2}{c}{{1-Day}} & \multicolumn{2}{c}{{1-Week}} & \multicolumn{2}{c}{{1-Month}}  \\
     \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
                 & MSE    & QLIKE  & MSE    & QLIKE  & MSE     & QLIKE  \\\midrule
        
                 & \multicolumn{6}{c}{{Panel B: Top 10\%}}  \\ \midrule
HAR$_M$          & 1.000   & 1.000  & 1.000  & 1.000  & 1.000   & 1.000  \\
GHAR$_M$         & 0.916  & 0.910   & 0.897  & 0.959  & 0.976$^*$  & 1.043  \\
GNNHAR1L$_M$     & 0.895  & 0.903   & 0.949  & 0.908  & 1.033   & 1.007  \\
GNNHAR2L$_M$     & 1.102  & 0.915   & 1.056  & 0.951  & 1.157   & 1.131  \\
GNNHAR3L$_M$     & 1.293  & 0.958   & 1.030  & 0.952  & 1.059   & 0.982  \\
HAR$_Q$          & 0.900  & 0.965   & 0.928  & 0.925  & 1.059   & 1.024  \\
GHAR$_Q$         & 0.852  & 0.867$^{\dagger}$  & 0.804$^*$ & 0.799$^*$ & 1.149   & 0.841$^*$ \\
GNNHAR1L$_Q$     & 0.834$^*$ & 0.879   & 0.841  & 0.848  & 1.143   & 0.955  \\
GNNHAR2L$_Q$     & 0.848  & 0.862$^*$  & 0.924  & 0.861  & 1.773   & 0.886  \\
GNNHAR3L$_Q$     & 0.868  & 0.882   & 1.205  & 0.909  & 1.483   & 0.973  \\\bottomrule
\end{tabular}

==> tables/var_1d_main.tex <==
\begin{tabular}{lcccc}
\toprule
& \multicolumn{2}{c}{{MSE}} & \multicolumn{2}{c}{{QLIKE}} \\
     \cmidrule(lr){2-3}\cmidrule(lr){4-5}
 & Ratio  & $p$-val &  Ratio & $p$-val \\
\midrule
% \multicolumn{5}{c}{Panel A: trained with MSE} \\\midrule
HAR$_M$          & 1.000 & $<$0.001  & 1.000 & $<$0.001\\
GHAR$_M$         & 0.927 & $<$0.001  & 0.983 & $<$0.001\\
GNNHAR1L$_M$     & 0.907 & $<$0.001  & 0.979 & $<$0.001\\
GNNHAR2L$_M$     & 1.063 & $<$0.001  & 0.977 & $<$0.001\\
GNNHAR3L$_M$     & 1.210 & $<$0.001  & 0.982 & $<$0.001\\\midrule
% \multicolumn{5}{c}{Panel B: trained with QLIKE} \\\midrule
HAR$_Q$          & 0.927 & $<$0.001  & 0.981 & $<$0.001\\
GHAR$_Q$         & 0.886 & $<$0.001  & 0.983 & $<$0.001\\
GNNHAR1L$_Q$     & 0.867 & 1.000     & 0.959 & 1.000 \\
GNNHAR2L$_Q$     & 0.879 & $<$0.001  & 0.962 & 0.001 \\
GNNHAR3L$_Q$     & 0.894 & $<$0.001  & 0.963 & $<$0.001\\
\bottomrule
\end{tabular}
